Testing Quantum Mechanics using Noisy Quantum Computers

We outline a proposal to test quantum mechanics in the high-complexity regime using noisy intermediate-scale quantum (NISQ) devices. The procedure involves simulating a non-Clifford random circuit, followed by its inverse, and then checking that the resulting state is the same as the initial state. We are motivated by the hypothesis that quantum mechanics is not fundamental, but instead emerges from a theory with less computational power, such as classical mechanics. This emergent quantum mechanics (EmQM) hypothesis makes the prediction that quantum computers will not be capable of sufficiently complex quantum computations. We show that quantum mechanics predicts that the fidelity of our procedure decays exponentially with circuit depth (due to noise in NISQ devices), while EmQM predicts that the fidelity will decay significantly more rapidly for sufficiently deep circuits, which is the experimental signature that we propose to search for. We estimate rough bounds for when possible signals of EmQM should be expected. Furthermore, we find that highly informative experiments should require only thousands qubits.

==> SM.tex <==

\section{Exponential Fidelity Decay via 2-design Twirling}
\label{app:twirl}

Given a gate independent noise assumption and 2-design\footnote{%
  We thank Alex Dalzell for pointing out that a 2-design approximation is sufficient, rather than a 4-design.}
  approximation,
  we can generalize the randomized benchmarking 2-design twirling argument \cite{tdesignRB} to our protocol.
Similar to the main texts, we find that quantum mechanics predicts an exponential fidelity decay [\eqnref{eq:f}].

We assume that the noise is gate and time independent,
  but it may depend on the position of the 2-qubit gate.
Therefore,\arxiv{ in the notation of \secref{sec:decay},}
  the noise channels are assumed to be the same for different 2-qubit gates $u_{t,i}$ and $u_{t',i}$
  acting on the same pair of qubits labeled by $i$:
  $\mathcal{N}_{u_{t,i}} = \mathcal{N}_{u_{t',i}}$.
However, we can allow the noise for the forward and backward circuits to be different.
As is also the case in the main text,
  it is not essential to assume that the noise only comes from 2-qubit error channels.

We also approximate each layer of 2-qubit gates $U_t$ as a 2-design.
Formally, this approximation is not justified
  since an approximate 2-design requires a $O(n^{1/D})$-depth $D$-dimensional circuit \cite{approximateTDesign}.
However, this approximation might be better than expected if we can instead think of it as
  only approximating the composition of $O(n^{1/D})$ layers of gates as a 2-design.
We do not consider this possibility here
  since it would complicate the definition of the noise channel $\mathcal{N}$ below.

To simplify the notation, we rewrite the Markovian fidelity \eqnref{eq:F model} from the main text as
\begin{equation}
  F_d = \Exp_{U_1, \ldots, U_d} \tr( \rho'_d \, \rho_d )
\end{equation}
  where
\begin{gather}
\begin{aligned}
  \rho'_d &\equiv (\Phi_{U_d^\dagger}^\dagger \!\circ\cdots\circ \Phi_{U_1^\dagger}^\dagger) (\rhof) \\
  \rho_d  &\equiv (\Phi_{U_d} \!\circ\cdots\circ \Phi_{U_1}) (\rhoi)
\end{aligned}
\end{gather}
  implicitly depend on $U_1, \ldots, U_d$, and
  $\Phi^\dagger$ is defined such that $\tr[\Phi^\dagger(\rho') \, \rho] = \tr[\rho' \, \Phi(\rho)]$.
Below we recursively integrate out one $U_t$ at a time by
  approximating each $U_t$ as an arbitrary Haar random unitary (or a unitary 2-design) on $n$ qubits:
\begin{align}
  F_d &= \Exp_{U_1, \ldots, U_d} \tr\!\left[ \mathcal{N}_d'^{\dagger}(\rho'_{d-1}) \, U_d^\dagger \mathcal{N}_d(U_d \rho_{d-1} U_d^\dagger) U_d \right] \label{eq:F1}\\
      &\sim \frac{\hat{F}_d-2^{-2n}}{1-2^{-2n}} \Exp_{U_1, \ldots, U_{d-1}} \tr\!\left[ \mathcal{N}_d'^\dagger(\rho'_{d-1}) \, \rho_{d-1} \right] + (1-\hat{F}_d) \frac{2^{-n}}{1-2^{-2n}} \tr \mathcal{N}_d'^\dagger(\rho'_{d-1}) \label{eq:F2}\\
      &\sim \left( \prod_{t=d'+1}^d \frac{\hat{F}_t-2^{-2n}}{1-2^{-2n}} \right) \Exp_{U_1, \ldots, U_{d'}}
         \tr\!\left[ \mathcal{N}_{d'}'^\dagger(\rho'_{d'-1}) \, U_{d'}^\dagger (\mathcal{N}'_{d'+1} \circ \mathcal{N}_{d'})(U_{d'} \rho_{d'-1} U_{d'}^\dagger) U_{d'} \right] \\
      &\quad\quad + \sum_{t=d'+1}^d (1-\hat{F}_t) \frac{2^{-n}}{1-2^{-2n}} \tr \mathcal{N}_t'^\dagger(\rho'_{t-1}) \nonumber\\
      &\sim \left( \prod_{t=1}^d \frac{\hat{F}_t-2^{-2n}}{1-2^{-2n}} \right) 
         \tr\!\left[ \mathcal{N}_1'^\dagger(\rhof) \, \rhoi \right] + \sum_{t=1}^d (1-\hat{F}_t) \frac{2^{-n}}{1-2^{-2n}} \tr \mathcal{N}_t'^\dagger(\rho'_{t-1}) \\
      &= \tr\!\left[ \mathcal{N}_1'^\dagger(\rhof) \, \rhoi \right] \, \prod_{t=1}^d \hat{F}_t + O(2^{-n}) \label{eq:F5}
\end{align}
$\mathcal{N}_t$ and $\mathcal{N}'_t$ are gate-independent noise channels of the forward and backward circuits:
  $\Phi_{U_t}(\rho) = \mathcal{N}_t(U_t \rho U_t^\dagger)$ and
  $\Phi_{U_t^\dagger}(\rho) = \mathcal{N}'_d(U_t^\dagger \rho U_t)$.
In the last line, we drop very small $O(2^{-n})$ terms.
$\hat{F}_t$ is the entanglement fidelity of $\mathcal{N}'_{t+1} \circ \mathcal{N}_t$ for $t=1,\ldots,d-1$,
  while $\hat{F}_d$ is just the entanglement fidelity of $\mathcal{N}_d$:
\begin{align}
  \hat{F}_t &= 2^{-2n} \tr\!\left(\mathcal{N}'_{t+1} \circ \mathcal{N}_t\right) &
  \hat{F}_d &= 2^{-2n} \tr \mathcal{N}_t \label{eq:hatF}\\
      &= 2^{-2n} \sum_{k',k} \left|\tr\!\left(E_{k'}'^{(t+1)} E_k^{(t)}\right)\right|^2 &
      &= 2^{-2n} \sum_{k} \left|\tr E_k^{(t)}\right|^2 \nonumber
\end{align}
$E_k^{(t)}$ and $E_{k'}'^{(t)}$ are Kraus operators of $\mathcal{N}_t$ and $\mathcal{N}'_t$; \emph{i.e.}
  $\mathcal{N}_t(\rho)  = \sum_k    E^{ (t)}_k    \rho\, E^{(t)\dagger}_k$ and
  $\mathcal{N}'_t(\rho) = \sum_{k'} E'^{(t)}_{k'} \rho\, E'^{(t)\dagger}_{k'}$.
Note that $\hat{F}_t = \hat{F}_{t+p}$ has periodicity $p$ since the circuit geometry is assumed to have periodicity $p$.

The entanglement fidelity of the composition $\mathcal{N}'_{t+1} \circ \mathcal{N}_t$ appears in \eqnref{eq:hatF}
  because coherent errors can cancel out.
For example, if $\mathcal{N}_t(\rho) = V \rho V^\dagger$ and $\mathcal{N}'_{t+1}(\rho) = V^\dagger \rho V$ for some unitary $V$,
   then the fidelity $F_d$ would not depend on the coherent error $V$.
This subtlety does not occur in randomized benchmarking \cite{noiseEstimation,tdesignRB,twirlRB}
  because randomized benchmarking uses a compactified inverse circuit.

\eqnref{eq:F5} is an exponential fidelity decay
  $F_d \sim \widetilde{F}_0 e^{-\lambda d}$
  with parameters
\begin{gather}
\begin{aligned}
  \widetilde{F}_0 &\approx \tr\!\left[ \mathcal{N}_1'^\dagger(\rhof) \, \rhoi \right] \frac{\tr \mathcal{N}_p}{\tr\!\left(\mathcal{N}'_{p+1} \circ \mathcal{N}_p\right)} \\
  \lambda &\approx -\frac{1}{p} \log \prod_{t=1}^p \hat{F}_t
\end{aligned} \label{eq:lambdaApp}
\end{gather}
  when $d$ is an integer multiple of the period $p$.

\eqnref{eq:lambdaApp} differs from \eqnref{eq:lambda} in the main text for two reasons:
  \eqnref{eq:lambda} neglected the fact that coherent errors in $\mathcal{N}'_{t+1} \circ \mathcal{N}_t$ can cancel out,
  while \eqnref{eq:lambdaApp} assumes that errors are gate-independent.
Unfortunately, the decay rate $\lambda$ in \eqnref{eq:lambdaApp} can not be written in terms of a product of 2-qubit gate fidelities
  [as in \eqnref{eq:lambda}]
  because $\mathcal{N}'_{t+1} \circ \mathcal{N}_t$ in the definition of $\hat{F}_t$
  involves two circuit layers with different positions of the 2-qubit gates.
If we were to make the rough approximation
  $2^{-2n} \tr\!\left(\mathcal{N}'_{t+1} \circ \mathcal{N}_t\right) \to
    2^{-4n} \tr\mathcal{N}'_{t+1} \tr \mathcal{N}_t$,
  then $\lambda$ in \eqnref{eq:lambdaApp} would simplify to \eqnref{eq:lambda}.

\section{Numerical Simulations}
\label{app:numerics}

In \figref{fig:simulation} we showed a simulation for a $5\times5$ grid of $n=25$ qubits
  using roughly Sycamore/Zuchongzhi-like \cite{GoogleSupremacy,ZuchongzhiAdvantage,ZuchongzhiAdvantage2} gates with gate-dependent errors.
\appsref{app:gates} and \ref{app:noise} specify the gate and noise models that we used.
\appref{app:Kraus} defines an optimized basis of Kraus operators that we used to minimize the amount of statistical sampling error.
All plots in the main text have statistical errors that are too small to be seen.
\appref{app:MPS simulation} specifies details used to produce the MPS data in \figref{fig:MPS}.

In \figref{fig:simulationApp}, we show a more detailed version of \figref{fig:simulation}
  showing a larger max circuit depth $d_\text{max}$.
At large depth, the fidelity $F_d$ saturates to $2^{-n}$,
  which will be too small to be experimentally observable for large $n \gtrsim 50$.
\figref{fig:simulationAppErr} shows the residual errors to the exponential decay fit.
The $\log(F_d) - \text{fit}$ residuals are dominated by the $2^{-n}$ saturation at large depth.
After subtracting off $2^{-n}$, we see that $F_d - 2^{-n}$ agrees with an exponential decay up to statistical errors.
The statistical errors of $F_d - 2^{-n}$ become very large once the fidelity decays to $2^{-n}$
  due to the $2^{-n}$ subtraction.

\begin{figure}
  \centering
  \subfloat[]{\includegraphics[width=.48\columnwidth]{simulationApp}} $\quad$
  \subfloat[\label{fig:simulationAppErr}]{\includegraphics[width=.48\columnwidth]{simulationAppErr}} \\
  \subfloat[\label{fig:circuit2d}]{\includegraphics[width=.6\columnwidth]{circuit2d}}
  \caption{%
    {\bf (a)} The same simulation data (black dots) as \figref{fig:simulation} (but for larger max depth $d_\text{max}$)
      showing the quantum mechanics prediction of
      the exponential fidelity $F_d$ decay
      for a $5\times5$ grid of $n=25$ noisy qubits.
    The fidelity $F_d$ saturates to $2^{-n}$ at large circuit depth $d$.
    Subtracting $2^{-n}$ from $F_d$ (green circles) leads to a continued exponential decay
      (at least until our simulation data becomes dominated by statistical errors).
    Also shown is a fit (blue line) to an exponential decay.
    {\bf (b)} With $2^{-n}$ subtracted, the fit residuals are dominated by statistical errors for our simulation of 10,000 Monte Carlo samples.
    Error bars denote one standard deviation (\emph{i.e.} 68\% confidence intervals).
    {\bf (c)} The period $p=4$ ordering of 2-qubit gates (green) applied to the $5\times5$ array of qubits.
  }\label{fig:simulationApp}
\end{figure}

To investigate the residuals with less statistical error,
  we also ran a simulation with less qubits
  (for which we can run significantly more Monte Carlo samples).
\figref{fig:simulationApp3x3} is similar to \figref{fig:simulationApp},
  but for a simulation of a $3\times3$ grid of $n=9$ qubits
  and a smaller average gate entanglement fidelity $f \approx 0.987$ (instead of $f \approx 0.993$).
In \figref{fig:simulationAppErr3x3},
  we see that residual errors to an exponential fit are very small when $F_d \gg 2^{-n}$.

\begin{figure}
  \centering
  \subfloat[]{\includegraphics[width=.48\columnwidth]{simulationApp3x3}} $\quad$
  \subfloat[\label{fig:simulationAppErr3x3}]{\includegraphics[width=.48\columnwidth]{simulationAppErr3x3}}
  \caption{%
    Same as \figref{fig:simulationApp}, but for a $3\times3$ grid of $n=9$ qubits,
      for which we obtained $8\times10^7$ Monte Carlo samples.
    Panel (b) shows that the residual errors of $F_d - 2^{-n}$ to an exponential fit are very small.
  }\label{fig:simulationApp3x3}
\end{figure}

\subsection{Gate Model}
\label{app:gates}

In our numerical simulations,
  we use gates that are somewhat similar to the Sycamore/Zuchongzhi gates \cite{GoogleSupremacy,ZuchongzhiAdvantage,ZuchongzhiAdvantage2}.
The gates are applied in the order shown in \figref{fig:circuit2d}.

Each 2-qubit gate $u_{t,i}$ is an iSWAP gate
  (rather than Sycamore/Zuchongzhi iSWAP-like gates \cite{GoogleSupremacy,ZuchongzhiAdvantage,ZuchongzhiAdvantage2})
\begin{equation}
  U_\text{iSWAP} = \begin{pmatrix}
                     1 &  0 &  0 & 0 \\
                     0 &  0 & -i & 0 \\
                     0 & -i &  0 & 0 \\
                     0 &  0 &  0 & 1
                   \end{pmatrix}
\end{equation}
  that is preceded by a pair of randomly chosen 1-qubit gates ($\sqrt{X}$, $\sqrt{Y}$, or $\sqrt{W}$) on two qubits,
  where $W = \frac{1}{\sqrt{2}} (X+Y)$.
Using $U_\text{iSWAP}^\dagger = U_\text{iSWAP} \, (Z \otimes Z)$,
  we decompose the inverse gate $u_{t,i}^\dagger$ as an iSWAP gate followed by a
  $\sqrt{X}^\dagger Z$, $\sqrt{Y}^\dagger Z$, or $\sqrt{W}^\dagger Z$ gate on each of the two qubits.

\subsection{Noise Model}
\label{app:noise}

In our numerical simulations,
  we use a generic error model with gate and position dependent errors.
Each iSWAP gate for each pair of qubits (labeled by $i$) has a unique noise channel.
And for each of the $n$ qubits, we apply a unique noise channel for each of six the 1-qubit gates
  ($\sqrt{X}$, $\sqrt{Y}$, $\sqrt{W}$, $\sqrt{X}^\dagger Z$, $\sqrt{Y}^\dagger Z$, and $\sqrt{W}^\dagger Z$).
Each noise channel is generated randomly.
None of our plots appear to differ qualitatively for different random instances of gate error channels.

One way to generate a random noise channel on a $d$-dimensional Hilbert space is to
  choose a set of $m$ Kraus operators as a Haar random $md \times d$ semi-unitary matrix $E_{ka,b}$
  (\emph{i.e.} $\sum_{ka} E_{ka,b'}^* E_{ka,b} = \delta_{b',b}$).
Then the noise channel is
\begin{equation}
  \mathcal{N}_m(\rho) \overset{\text{rand}}{=} \sum_{k=1}^m E_k \rho E_k^\dagger
\end{equation}
In order to cover the set of all noise channels, one must choose $m=d^2$.
However, for $d=4$ or larger, this leads to a distribution of noise channels that is
  strongly concentrated near the depolarizing channel.
In order to obtain a broader but still generic distribution of noise channels,
  we generate each random noise channel as an average of the above random noise channel for $m=1,2,\ldots,d^2$:
\begin{equation}
  \mathcal{N}_\text{rand}(\rho) \overset{\text{rand}}{=} d^{-2} \sum_{m=1}^{d^2} \mathcal{N}_m(\rho)
\end{equation}

We also apply a randomly-chosen coherent error for each gate.
For a $d$-dimensional Hilbert space, we generate coherent error channels using a random unitary that is generated by
\begin{equation}
  U_p \overset{\text{rand}}{=} e^{i \sqrt{\frac{p}{d-1}} H^\text{Gauss}_\text{rand}}
\end{equation}
  where $H^\text{Gauss}_\text{rand}$ is a complex standard Gaussian random matrix
  and $p$ tunes the infidelity.

Each noise channel is then generated via
\begin{equation}
  \mathcal{N}_p(\rho) \overset{\text{rand}}{=} U_{p''/2} \left[ \left(1-\tfrac{p'}{2}\right) \rho + \tfrac{p'}{2} \, \mathcal{N}_\text{rand}(\rho) \right] U_{p''/2}^\dagger \label{eq:noise}
\end{equation}
  where $p'$ and $p''$ are randomly chosen between $p/\sqrt{2}$ and $\sqrt{2} \,p$.
The entanglement fidelity of $\mathcal{N}_p$ is roughly $1-p$.

We randomly generated the 2-qubit iSWAP noise channel using $\mathcal{N}_{p_2}$,
  while the 1-qubit noise channels were randomly generated using $\mathcal{N}_{p_1}$,
  with $p_1 = 0.1 p_2$.
For \figsref{fig:simulation}, \ref{fig:MPS}, and \ref{fig:simulationApp}, we used $p_2 = 0.005$.
For \figref{fig:simulationApp3x3}, we used $p_2 = 0.01$.

\subsection{Simulation Algorithm Details}
\label{app:Kraus}

We simulate the fidelity in \eqnref{eq:F model} by Monte Carlo (MC) sampling the density matrices and quantum channels
  such that only two wavefunctions are stored in memory: one from $\rhoi$ and the other from $\rhof$.
To reduce the amount of statistical error,
  we sample the density matrices and quantum channels such that each MC sample has the same average entanglement fidelity.

That is, $\rhoi$ and $\rhof$ are uniformly sampled from unnormalized wavefunctions
  $\ket{\psi^\text{init}_k}$ and $\ket{\psi^\text{fin}_k}$:
\begin{equation}
\begin{aligned}
  \rhoi &= \Exp_k \, \ket{\psi^\text{init}_k} \bra{\psi^\text{init}_k} \\
  \rhof &= \Exp_k \, \ket{\psi^\text{fin}_k} \bra{\psi^\text{fin}_k}
\end{aligned} \label{eq:wavefunctions}
\end{equation}
  which are chosen to have the same fidelity:
\begin{equation}
\begin{aligned}
  \braket{0|\psi^\text{init}_k} &= \braket{0|\psi^\text{init}_{k'}} \\
  \braket{0|\psi^\text{fin}_k} &= \braket{0|\psi^\text{fin}_{k'}}
\end{aligned} \label{eq:wavefunctions constraint}
\end{equation}
In \eqnref{eq:wavefunctions}, $\tExp_k \equiv n_k^{-1} \sum_k$
  denotes an expectation value over $n_k$ uniformly random $k$.
Similarly, the quantum channels $\Phi_u$ are rewritten using a Kraus decomposition
\begin{equation}
  \Phi_u(\rho) = \Exp_k E^{(u)}_k \rho \, E^{(u)\dagger}_k
\end{equation}
  (with nonstandard normalization due to the $\Exp_k$)
  such that each Kraus operator has the same trace:
\begin{equation}
  \tr E^{(u)}_k = \tr E^{(u)}_{k'} \label{eq:Kraus constraint}
\end{equation}
This implies that each Kraus operator has the same entanglement fidelity as $\Phi_u$:
  $f_u = 2^{-2m} \tr E^{(u)}_k \tr E^{(u)\dagger}_k$
  where $E^{(u)}_k$ is a $2^m \times 2^m$ matrix.
With this optimization,
  for a given sequence of unitaries $U_1,\ldots,U_d$,
  each MC sample has the approximately the same fidelity,
  which leads to a significant reduction in MC statistical error.

We only require that these special wavefunctions and Kraus operators obey linear constraints
  [\eqnref{eq:wavefunctions constraint} and \eqref{eq:Kraus constraint}].
They can therefore be obtained from another decomposition (\emph{e.g.} an eigendecomposition),
  $\rho = \tExp_{\tilde{k}} \ket{\widetilde{\psi}_{\tilde{k}}} \bra{\widetilde{\psi}_{\tilde{k}}}$ or
  $\Phi(\rho) = \tExp_{\tilde{k}} \widetilde{E}_{\tilde{k}} \rho \widetilde{E}^\dagger_{\tilde{k}}$,
  via a unitary transformation $V_{k,\tilde{k}}$ that rotates the vector
  $v_{\tilde{k}} = \braket{0|\widetilde{\psi}_{\tilde{k}}}$ (or $v_{\tilde{k}} = \tr \widetilde{E}_{\tilde{k}}$)
  to $\sum_{\tilde{k}} V_{k,\tilde{k}} v_{\tilde{k}} = \sqrt{f}$
  for some constant fidelity $f>0$.
That is, $\ket{\psi_k} = V_{k,\tilde{k}} \ket{\widetilde{\psi}_{\tilde{k}}}$
  and $E_k = V_{k,\tilde{k}} \widetilde{E}_{\tilde{k}}$.

Each MC sample for a sequence of fidelities $F_d$ with $d=0,\ldots,d_\text{max}$ is then obtained as follows:
\begin{enumerate}
  \item sample initial forward circuit wavefunction: $\ket{\psi}  \leftarrow \ket{\psi^\text{init}_k}$ for uniformly random $k$
  \item sample final   backward circuit wavefunction: $\ket{\psi'} \leftarrow \ket{\psi^\text{fin}_k}$ for uniformly random $k$
  \item foreach circuit depth $d=1,\ldots,d_\text{max}$:
  \begin{enumerate}
    \item foreach 2-qubit gate position $i$:
    \begin{enumerate}
      \item randomly sample an allowed gate: $u_{d,i}$
      \item apply random Kraus operator for forward gate: $\ket{\psi}  \leftarrow E^{(u_{d,i})}_k \ket{\psi}$
            for uniformly random $k$
      \item apply random Kraus operator for backward gate: $\ket{\psi'} \leftarrow E^{(u_{d,i}^\dagger)\dagger}_k \ket{\psi'}$
            for uniformly random $k$
    \end{enumerate}
    \item obtain fidelity sample: $F_d \leftarrow |\braket{\psi' | \psi}|^2$
  \end{enumerate}
\end{enumerate}

\subsection{MPS Simulation}
\label{app:MPS simulation}

In \figref{fig:MPS}, we showed a MPS simulation of our protocol with noisy gates for a chain of 24 qubits.
We used the same noise and gate models and sampling algorithm as in \figref{fig:simulation},
  \emph{i.e.} the models in \appsref{app:gates} and \ref{app:noise} and algorithm in \appref{app:Kraus}.

Random gates, SPAM errors, and random Kraus operators are randomly sampled
  as described in \appref{app:Kraus}.
However, a subtlety results from the fact that the MPS simulation introduces non-linear truncation errors.
When there is no truncation error, as in the quantum mechanics prediction (blue in \figref{fig:MPS}),
  then changing the Kraus operator basis $E_k \to V_{k,k'} E_{k'}$
  does not affect the fidelity.
But when there is truncation error, the choice of Kraus operator basis will affect the simulation result.
Typically, Kraus operators that are more like measurement operators will reduce the amount of entanglement,
  which decreases the amount of truncation error in later truncation steps.
Alternatively, Kraus operators that are closer to unitary operators
  typically result in a larger truncation error.
We use the Kraus basis defined in \appref{app:Kraus} for the MPS simulation,
  which is a nice choice because all of the Kraus operators behave similarly with similar fidelity.

\section{Drift}
\label{app:drift}

While iterating our protocol many times (\emph{e.g.} over the course of hours)
  to obtain a large number of samples,
  slow temperature fluctuations (and other causes) can result in miscalibrations (and other complications)
  that slowly drift \cite{drift} over time.
As a result, the effective error channel of each gate can change over time,
  resulting in slowly-varying gate fidelities \cite{cycleBenchmarking} for different samples.
To mitigate issues resulting from drift,
  our protocol samples a random circuit depth $d$ for each sample.
If circuit depth was instead sampled in increasing order,
  then drift could potentially cause the gate fidelity to decrease over time,
  which could then lead to a fidelity $F_d$ decay that could be mistaken for the EmQM signature.
By randomly sampling circuit depth,
  we can show that the effect of slow temporal drift
  can only cause the exponential fidelity $F_d$ decay rate to slightly decrease with circuit depth $d$,
  rather than increase as for EmQM.
This occurs because if the drift occurs much slower than the time scale to sample all circuit depths,
  then for larger depth, the fidelity $F_d$ is dominated by rare samples with rare but higher gate fidelities (due to rare drifts),
  while at smaller depth the fidelity is dominated by typical gate fidelities.
As such, the effects of drift are unlikely to be confused with the EmQM signature.

To see this more explicitly, we can consider the following toy model.
Assume that quantum mechanics is correct and
  suppose that temporal drifts occur over a time scale that is much longer than the time it takes to run a single sample in our protocol.
Then suppose that due to drift, the probability that a sample measures a zero state is the following time-dependent fidelity:
\begin{equation}
  F_d(t) = e^{-\lambda(t) d}
\end{equation}
Similar to \eqnref{eq:F},
  the fidelity decays exponentially with circuit depth $d$
  (although we neglect SPAM errors, \emph{i.e.} the $\widetilde{F}_0$ factor, for simplicity).
However, the fidelity also depends on time
  since the exponential decay rate $\lambda(t)$ is time-dependent due to slow time-dependent drifts.

To gain intuition, suppose that the fidelity decay rate $\lambda(t)$ drifts between $\lambda_1$ and $\lambda_2$ with a uniform probability distribution in-between.
Then the average probability that a sample measures a zero state is the average fidelity:
\begin{equation}
\begin{aligned}
  F_d &= \frac{1}{\lambda_2 - \lambda_1} \int_{\lambda_1}^{\lambda_2} e^{-\lambda d} \, \mathrm{d}\lambda \\
    &= \frac{1}{d} \frac{e^{-\lambda_1 d} - e^{-\lambda_2 d}}{\lambda_2 - \lambda_1} 
\end{aligned} \label{eq:drift12}
\end{equation}
See \figref{fig:drift} for an example plot.
At small depth, $F_d \approx e^{-\lambda d}$ where $\lambda = \frac{1}{2} (\lambda_1 + \lambda_2)$,
  while at large depth $F_d \approx (\lambda_2 - \lambda_1)^{-1} \frac{1}{d} \, e^{-\lambda_1 d}$.
Thus the fidelity decays slower at larger depth (in contrast to the EmQM signature)
  since $\lambda_1 < \lambda$.

\begin{figure}
  \centering
  \includegraphics[width=.35\columnwidth]{drift} \\
  \caption{%
    An exponential fidelity decay $F_d = e^{-\lambda d}$ without drift (blue)
      vs a fidelity decay with drift (orange) [\eqnref{eq:drift12} with $\lambda_1 = \frac{2}{3}\lambda$ and $\lambda_2 = \frac{4}{3}\lambda$].
    Drift only causes the fidelity to decay slightly slower at larger depth,
      which can not be mistaken for the EmQM signature [shown in \figref{fig:decay}].
  }\label{fig:drift}
\end{figure}

Now consider a general probability distribution $P(\lambda)$ of fidelity decay rates $\lambda(t)$ after time averaging.
Then the fidelity is $F_d = \int_\lambda e^{-\lambda d}$
  where $\int_\lambda f(\lambda) \equiv \int_0^\infty f(\lambda) P(\lambda) \,\mathrm{d}\lambda$
  averages over the different decay rates.
In this general setting, we can also show that the fidelity decays slower at larger depth.
The exponential decay rate near a given depth is
  the average of $\lambda(t)$:
\begin{equation}
  - \partial_d \log F_d
    = \braket{\lambda}_d
        \quad\text{where}\quad \braket{f(\lambda)}_d \equiv \frac{\int_\lambda f(\lambda) \, e^{-\lambda d}}{\int_\lambda e^{-\lambda d}}
\end{equation}
The slope of the curve $\log F_d$ is thus $-\braket{\lambda}_d$.
The derivative of this slope is then the variance of $\lambda(t)$:
\begin{equation}
  -\partial_d \braket{\lambda}_d
    = \braket[\big]{(\lambda - \braket{\lambda}_d)^2}_d
\end{equation}
Since the above variance is always positive, the derivative of the slope of $\log F_d$ vs $d$ is always positive.
This implies that the fidelity decays slower at larger depth than slower depth,
  which is opposite of the EmQM signature.

\arxiv{\newpage}
\section{MPS}
\label{app:MPS}

In \arxivPR{\secref{sec:MPS}}{the main text}, we considered the time evolution of matrix product states (MPS) \cite{MPS} with fixed bond dimension
  as an (incomplete) toy model of emergent quantum mechanics (EmQM) in one spatial dimension.
And in \appref{app:realism},
  we explain how and why tensor networks are not ruled out by Bell experiments.
However, we do not consider MPS to be a legitimate model of EmQM because
  it is currently not known how (or if it is possible) to generalize MPS algorithms to a three-dimensional local classical theory
  that could be compatible with previous experiments.
We elaborate on this point below.

One of the hallmarks of MPS is the canonical form,
  which allows one to calculate the expectation value of a local operator near some position $x$
  in terms of only the tensors near $x$.
When generalizing MPS to higher dimensions,
  this sense of canonical form can either be retained,
  as is done for isometric tensor networks \cite{IsometricTN,2dDMRG,canonicalPEPS};
  or the canonical form can be dropped,
  as is done for projected entangled pair states (PEPS) \cite{OrusTN};
  or the canonical form can be replaced with something new (but less constraining),
  such as a weighted trace gauge (WTG) \cite{EvenblyCanonical}.

When the canonical form is retained \cite{IsometricTN,2dDMRG,canonicalPEPS},
  a local update algorithm to time evolve the tensor network is known \cite{IsometricTN}.
However, the algorithm does not quite yet yield a local classical theory since the update algorithm has to iteratively sweep across the tensor network.
This is similar to many MPS algorithms, such as TDVP \cite{TDVP},
  which time evolve a length-$L$ chain by performing a forward sweep to update the tensors at
  sites $i$ and $i+1$ for $i=1,2,\ldots,L-1$,
  followed by a backward sweep with $i=L-1,L-2,\ldots,1$.
It would be incredibly unnatural if the time evolution of the universe sweeps across space in this serial (rather than parallel) manner.
Therefore, we expect an EmQM theory to have the form of a local classical theory:
  \emph{i.e.} a (possibly continuous) cellular automaton
  for which the local updates are performed in parallel for all sites at once.
Nevertheless, we expect that it is possible to parallelize the time-evolving isometric tensor network algorithm \cite{IsometricTN}
  into a continuous cellular automaton,
  \emph{e.g.} by using ideas from \refcite{ParallelDMRG}.

However, there is a more severe issue that is also shared with MPS:
  between certain pairs of well-separated spatial disks of radius $\ell$,
  isometric tensor networks \cite{IsometricTN} and canonical PEPS \cite{canonicalPEPS,2dDMRG}
  can only represent wavefunctions that have a bounded amount of entanglement between the two regions.
In particular, the mutual information $I$ between certain pairs of regions is bounded by the log of the bond dimension $\chi$:
  $I < \log \chi$.
Even a large bond dimension $\chi = 1024$ is only large enough to encode 10 bell pairs between the two regions.
Unless $\chi$ is extraordinarily large,
  this is incompatible with many experiments, including the recent quantum advantage experiments
  \cite{GoogleSupremacy,ZuchongzhiAdvantage,ZuchongzhiAdvantage2,PhotonAdvantage}.\footnote{%
  However, extra spatial dimensions could be used to solve this bounded entanglement problem \cite{SlagleTensor}.}

An EmQM theory should allow the mutual information to diverge with the length scale $\ell$,
  so that quantum mechanics with highly-entangled quantum states can emerge in the large length limit $\ell \to \infty$.

On the other hand, PEPS do appear to be possibly powerful enough to represent wavefunctions
  that are sufficiently entangled to be compatible with current experimental observations.
For example, the mutual information bound for PEPS diverges linearly with the length scale: $I < O(\ell \log \chi)$.
Furthermore, due to their unconstrained nature,
  unitary circuits can easily be embedded into a PEPS in order to represent high-complexity wavefunctions.
This is especially true if the PEPS exists in extra spatial dimensions and/or
  if physical qubits are separated by large distances in the lattice of tensors,
  as in \figref{fig:PEPS}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{PEPS} \\
  \caption{%
    A PEPS with physical qubits (dangling red lines) separated by many
      unimportant qubits (dangling gray lines), which we consider unimportant after coarse-graining.
    Black dots represent tensors which are contracted along the black lines.
    We see that the PEPS can easily represent many well-separated by Bell states
      by threading their entanglement along the blue lines.
    Furthermore, unitary circuits can be embedded into the PEPS
      (with unitary gates encoded in tensor pairs highlighted in green)
      to encode high-complexity states.
  }\label{fig:PEPS}
\end{figure}

However, we are not aware of any time-evolving PEPS algorithms that could be written as a local classical theory.
For example, PEPS update algorithms typically require calculating environment tensors,
  which involve a non-local contraction of the entire tensor network,
  for which non-local approximate algorithms are necessary \cite{AlgorithmsPEPS,GradientPEPS}.

However, the biggest challenge in formulating an EmQM theory using a tensor network algorithm is that so far,
  no (local or nonlocal) time-evolving tensor network algorithm has been shown to be robust enough to create high-complexity states
  (\emph{e.g.} those created during the quantum advantage experiments \cite{GoogleSupremacy,ZuchongzhiAdvantage,ZuchongzhiAdvantage2,PhotonAdvantage})
  with fixed bond dimension.
With sufficiently large bond dimension, most tensor network algorithms can simulate essentially anything.
However in EmQM, we would like to imagine that the bond dimension is fixed and not too large.
Instead, it is the distance between physical qubits and time over which the dynamics occurs that is large,
  and it is over these extremely large scales that perhaps quantum mechanics could emerge.

\newpage
\section{Bell's Theorem and Tensor/Neural Networks}
\label{app:Bell}

Bell's theorem \cite{BellTheorem} and its conceptually simpler\footnote{%
    The GHZ variant is simpler in the sense that every measurement outcome is fixed according to quantum mechanics
      and simultaneously inconsistent with a local hidden variable theory.
    In contrast, Bell's original theorem only establishes a probabilistic Bell inequality.
    However, the GHZ variant involves three qubits instead of two.}
  GHZ variant \cite{BellGHZ,MerminBellGHZ,PhotonBellGHZ} show that
  local hidden variable theories are incompatible with quantum mechanics.
In \appref{app:GHZ}, we review the GHZ variant.
In \appref{app:realism}, we then discuss why tensor networks and neural networks
  are not local hidden variable theories [spoiler: \eqsref{eq:realism} and \eqref{eq:local realism} are not satisfied]
  and can therefore bypass Bell's theorem (and its variants).
Invoking a superdeterminism \cite{superdeterminism} loophole \cite{bellLoopholes} is not necessary.

\subsection{Review: GHZ Variant of Bell's Theorem}
\label{app:GHZ}

Writing the 3-qubit GHZ state in the ZZZ, YYX, and XXX basis yields:
\begin{align}
  \ket{\psi} &= \tfrac{1}{\sqrt{2}} \ket{+_z +_z +_z} + \tfrac{1}{\sqrt{2}} \ket{-_z -_z -_z} & ZZZ \text{ basis} \nonumber\\
             &= \tfrac{1}{2} \ket{-_y -_y -_x} + \tfrac{1}{2} \ket{-_y +_y +_x}
              + \tfrac{1}{2} \ket{+_y -_y +_x} + \tfrac{1}{2} \ket{+_y +_y -_x} & YYX \text{ basis} \label{eq:GHZ}\\
             &= \tfrac{1}{2} \ket{+_x +_x +_x} + \tfrac{1}{2} \ket{+_x -_x -_x}
              + \tfrac{1}{2} \ket{-_x +_x -_x} + \tfrac{1}{2} \ket{-_x -_x +_x} & XXX \text{ basis} \nonumber
\end{align}
$\ket{\psi}$ takes a similar permuted form in the YXY and XYY basis.
We use the following notation for the qubit states
\begin{gather}
\begin{aligned}
  \ket{\pm_x} &= \tfrac{1}{\sqrt{2}} \ket{+_z} \pm \tfrac{1}{\sqrt{2}} \ket{-_z} \\
  \ket{\pm_y} &= \tfrac{1}{\sqrt{2}} \ket{+_z} \pm \tfrac{i}{\sqrt{2}} \ket{-_z} \\
\end{aligned}
\end{gather}
  which are eigenstates of the Pauli operators:
  $\hat{\sigma}^\mu \ket{\pm_\mu} = \pm \ket{\pm_\mu}$.
In this Appendix, operators will always be denoted with a hat.
Note that the GHZ state has a fixed measurement outcome for the $\hat{Y}_1 \hat{Y}_2 \hat{X}_3$ and $\hat{X}_1 \hat{X}_2 \hat{X}_3$ operators
  (along with permutations)
\begin{equation}
\begin{aligned}
\braket{\psi|\hat{Y}_1 \hat{Y}_2 \hat{X}_3|\psi} &= -1\\
\braket{\psi|\hat{X}_1 \hat{X}_2 \hat{X}_3|\psi} &= +1
\end{aligned} \label{eq:quantum exp}
\end{equation}
$\hat{X}_i$ denotes the $\hat{\sigma}^x$ Pauli operator acting on the $i^\text{th}$ qubit,
  and similar for $\hat{Y}_i$ and $\hat{Z}_i$.

In a hidden variable theory\footnote{%
    Other definitions of hidden variable theories exist in the literature \cite{AaronsonHiddenVariable}.
    We are reviewing the definition as used in Bell's theorem.},
  measurement outcomes only depend on a hidden classical variable $h$,
  which has a probability density $P(h)$.
The measurement outcome due to measuring a qubit $i$ in the X, Y, or Z basis can then be written as:
\begin{align}
  X_i(h) &= \pm1 \nonumber\\
  Y_i(h) &= \pm1 \label{eq:realism}\\
  Z_i(h) &= \pm1 \nonumber
\end{align}
Therefore, the quantum expectation values reduce to classical expectation values:
\begin{align}
  \braket{\psi|\hat{X}_i|\psi} &= \int_h P(h) \, X_i(h) \nonumber\\
  \braket{\psi|\hat{Y}_i|\psi} &= \int_h P(h) \, Y_i(h) \\
  \braket{\psi|\hat{Z}_i|\psi} &= \int_h P(h) \, Z_i(h) \nonumber
\end{align}
In a \emph{local} hidden variable theory, measuring qubit $i$ can not affect the measurement outcome of qubit $j$
  if qubit $j$ is far away and measured immediately after qubit $i$.
Therefore, for space-like separated measurements in a local hidden variable theory, the multi-point quantum expectation values
  also reduce to analogous classical expectation values; in particular:
\begin{equation}
\begin{aligned}
  \braket{\psi|\hat{Y}_1 \hat{Y}_2 \hat{X}_3|\psi} &= \int_h P(h) \, Y_1(h) Y_2(h) X_3(h) \\
  \braket{\psi|\hat{X}_1 \hat{X}_2 \hat{X}_3|\psi} &= \int_h P(h) \, X_1(h) X_2(h) X_3(h)
\end{aligned} \label{eq:local realism}
\end{equation}

To obtain a contradiction with quantum theory, note that
  \eqsref{eq:quantum exp},
  \eqref{eq:realism},
  \eqref{eq:local realism},
  and permutations imply that
\begin{align}
  Y_1(h) Y_2(h) X_3(h) &= Y_1(h) X_2(h) Y_3(h) = X_1(h) Y_2(h) Y_3(h) = -1 \label{eq:local YYZ} \\
  X_1(h) X_2(h) X_3(h) &= +1 \label{eq:local XXX}
\end{align}
for all hidden variables $h$ (with $P(h) \neq 0$).
However, $X_1(h) X_2(h) X_3(h)$ can be rewritten using \eqnref{eq:local YYZ}
\begin{gather}
\begin{aligned}
  X_1(h) X_2(h) X_3(h) &= [Y_1(h) Y_2(h) X_3(h)] \, [Y_1(h) X_2(h) Y_3(h)] \, [X_1(h) Y_2(h) Y_3(h)] \\
    &= [-1] [-1] [-1] = -1
\end{aligned} \label{eq:local XXX'}
\end{gather}
since $Y_i(h)^2 = 1$.
The above \eqnref{eq:local XXX'} contradicts \eqnref{eq:local XXX}.
This shows that quantum mechanics can not be described by a local hidden variable theory.

\subsection{Tensor and Neural Networks}
\label{app:realism}

Tensor networks and neural networks might seem like hidden variable theories.
However, neither are local hidden variable theories
  and are therefore not ruled out by Bell experiments.
The primary issue is that observables are not well-defined in terms of hidden variables, as in \eqnref{eq:realism},
  in tensor or neural networks.

Furthermore, in the limit of infinite bond dimension or number of training parameters,
  tensor and neural networks can simulate quantum mechanics exactly \cite{CiracTensorRev,StoudenmireLimits,PollmannNeural},
  which implies that Bell's theorem must not be violated in that limit.
If an exact tensor or neural network (or other EmQM theory in an exact limit) were to simulate a Bell experiment,
  then there would be no sense of local realism.
That this, after the observers measured their qubits,
  the EmQM theory would be encoding a wavefunction that consists of a superposition of measurement outcomes,
  as predicted by Schr\"{o}dinger's equation.
As emphasized in the many-worlds interpretation of quantum mechanics,
  the wavefunction would then approximately consist of multiple ``branches'' that evolve independently in superposition
  since they are extremely unlikely to interfere with each other\footnote{%
    This assumes that the observers (including the surrounding environment) consist of many chaotic degrees of freedom, which is certainly true for human observers.}.
In an actual non-exact EmQM theory,
  only a limited number of wavefunction branches could be retained.
Therefore, \emph{after} the measurements took place,
  an EmQM theory would eventually be forced to randomly drop wavefunction branches
  (especially if many Bell measurements are performed).
As long as only valid branches are retained and branches are dropped with the correct probability,
  the Bell experiments would not notice deviations from quantum mechanics.
In a matrix product state (MPS) tensor network,
  dropping a branch could be achieved by a special random (or pseudo-random) truncation of a bond dimension.

\subsubsection{GHZ Example}

For example, the 3-qubit GHZ state from \eqnref{eq:GHZ} can easily be encoded in a
  matrix product state (MPS) tensor network in the ZZZ basis:
\begin{align}
  \ket{\psi} &= \sum_{a_1,a_2,a_3,\alpha,\beta=0,1} A_{a_1,\alpha} \, B_{\alpha,a_2,\beta} \, C_{\beta,a_3}
                \ket{a_1a_2a_3} \\
  A_{a_1,\alpha} &= \delta_{a_1,\alpha} \nonumber\\
  B_{\alpha,a_2,\beta} &= 2^{-1/2} \delta_{\alpha,a_2,\beta} \\
  C_{\beta,a_3} &= \delta_{\beta,a_3} \nonumber
\end{align}
  where $(a_1,a_2,a_3)$ index states in the Z basis ($\ket{0} = \ket{+_z}$ and $\ket{1} = \ket{-_z}$)
  and $(\alpha,\beta)$ are virtual indices.
$\delta$ is the Kronecker delta, with $\delta_{a,b,c} = 1$ if $a=b=c$ else $\delta_{a,b,c} = 0$.

One could attempt to map the above tensor network to a hidden variable theory by defining the hidden variable as
  the physical and virtual indices: $h=(a_1,a_2,a_3,\alpha,\beta)$.
Then the Z-basis measurements obey the analogs of Eqs.\,(\ref{eq:realism}--\ref{eq:local realism}) with
  $P(h) = \frac{1}{2} \delta_{a_1,a_2,a_3,\alpha,\beta}$ and $Z_i(h) = (-1)^{a_i}$.
However, there is no choice of $X_i(h)$ and $Y_i(h)$ that is also consistent with Eqs.\,(\ref{eq:realism}--\ref{eq:local realism}).\footnote{%
  One might alternatively imagine adding $\alpha'$ and $\beta'$ to the hidden variable in order to account for
    virtual indices for a bra state.
  However, this does not help turn the tensor network into a local hidden variable theory.}

Neural networks also fail to be a local hidden variable theory in a similar way.

